Deep Hawkes Process for High-Frequency Market Making

High-frequency market making is a liquidity-providing trading strategy that simultaneously generates many bids and asks for a security at ultra-low latency while maintaining a relatively neutral position. The strategy makes a profit from the bid-ask spread for every buy and sell transaction, against the risk of adverse selection, uncertain execution and inventory risk. We design realistic simulations of limit order markets and develop a high-frequency market making strategy in which agents process order book information to post the optimal price, order type and execution time. By introducing the Deep Hawkes process to the high-frequency market making strategy, we allow a feedback loop to be created between order arrival and the state of the limit order book, together with self- and cross-excitation effects. Our high-frequency market making strategy accounts for the cancellation of orders that influence order queue position, profitability, bid-ask spread and the value of the order. The experimental results show that our trading agent outperforms the baseline strategy, which uses a probability density estimate of the fundamental price. We investigate the effect of cancellations on market quality and the agent's profitability. We validate how closely the simulation framework approximates reality by reproducing stylised facts from the empirical analysis of the simulated order book data.

==> src/LSTM.tex <==
\newcommand{\empt}[2]{$#1^{\langle #2 \rangle}$}
\begin{figure}[H]
\centering
\begin{tikzpicture}[
    % GLOBAL CFG
    font=\sf \scriptsize,
    >=LaTeX,
    % Styles
    cell/.style={% For the main box
        rectangle, 
        rounded corners=5mm, 
        draw,
        very thick,
        },
    operator/.style={%For operators like +  and  x
        circle,
        draw,
        inner sep=-0.5pt,
        minimum height =.2cm,
        },
    function/.style={%For functions
        ellipse,
        draw,
        inner sep=1pt
        },
    ct/.style={% For external inputs and outputs
        circle,
        draw,
        line width = .75pt,
        minimum width=1cm,
        inner sep=1pt,
        },
    gt/.style={% For internal inputs
        rectangle,
        draw,
        minimum width=4mm,
        minimum height=3mm,
        inner sep=1pt
        },
    mylabel/.style={% something new that I have learned
        font=\scriptsize\sffamily
        },
    ArrowC1/.style={% Arrows with rounded corners
        rounded corners=.25cm,
        thick,
        },
    ArrowC2/.style={% Arrows with big rounded corners
        rounded corners=.5cm,
        thick,
        },
    ]

%Start drawing the thing...    
    % Draw the cell: 
    \node [cell, minimum height =4cm, minimum width=6cm] at (0,0){} ;

    % Draw inputs named ibox#
    \node [gt] (ibox1) at (-2,-0.75) {$\sigma$};
    \node [gt] (ibox2) at (-1.5,-0.75) {$\sigma$};
    \node [gt, minimum width=1cm] (ibox3) at (-0.5,-0.75) {tanh};
    \node [gt] (ibox4) at (0.5,-0.75) {$\sigma$};

   % Draw opérators   named mux# , add# and func#
    \node [operator] (mux1) at (-2,1.5) {$\times$};
    \node [operator] (add1) at (-0.5,1.5) {+};
    \node [operator] (mux2) at (-0.5,0) {$\times$};
    \node [operator] (mux3) at (1.5,0) {$\times$};
    \node [function] (func1) at (1.5,0.75) {tanh};

    % Draw External inputs? named as basis c,h,x
    \node[ct] (c) at (-4,1.5)  {$c_{t-1}$};
    \node[ct] (h) at (-4,-1.5) {$h_{t-1}$};
    \node[ct] (x) at (-2.5,-3) {$x_{t}$};

    % Draw External outputs? named as basis c2,h2,x2
    \node[ct] (c2) at (4,1.5)  {$c_{t}$};
    \node[ct] (h2) at (4,-1.5) {$h_{t}$};
    \node[ct] (x2) at (2.5,3)  {$h_{t}$};

% Start connecting all.
    %Intersections and displacements are used. 
    % Drawing arrows    
    \draw [ArrowC1] (c) -- (mux1) -- (add1) -- (c2);

    % Inputs
    \draw [ArrowC2] (h) -| (ibox4);
    \draw [ArrowC1] (h -| ibox1)++(-0.5,0) -| (ibox1); 
    \draw [ArrowC1] (h -| ibox2)++(-0.5,0) -| (ibox2);
    \draw [ArrowC1] (h -| ibox3)++(-0.5,0) -| (ibox3);
    \draw [ArrowC1] (x) -- (x |- h)-| (ibox3);

    % Internal
    \draw [->, ArrowC2] (ibox1) -- (mux1);
    \draw [->, ArrowC2] (ibox2) |- (mux2);
    \draw [->, ArrowC2] (ibox3) -- (mux2);
    \draw [->, ArrowC2] (ibox4) |- (mux3);
    \draw [->, ArrowC2] (mux2) -- (add1);
    \draw [->, ArrowC1] (add1 -| func1)++(-0.5,0) -| (func1);
    \draw [->, ArrowC2] (func1) -- (mux3);

    %Outputs
    \draw [-, ArrowC2] (mux3) |- (h2);
    \draw (c2 -| x2) ++(0,-0.1) coordinate (i1);
    \draw [-, ArrowC2] (h2 -| x2)++(-0.5,0) -| (i1);
    \draw [-, ArrowC2] (i1)++(0,0.2) -- (x2);

\end{tikzpicture}
\end{figure}


\begin{eqnarray}
\label{equ:lstm}
\begin{aligned}

\!&\Bz_t \ &= \ g \left( \BW_{\Bz} \ \Bx_t \    + \ \BU_{\Bz} \ \By_{t-1} \  + \
   \Bb_{\Bz}\right) & \text{cell input} \label{Arr:eq_start:standard_LSTM_forward} \\
\Bi_t \ &= \ \sigma \left( \BW_{\Bi} \ \Bx_t \   + \ \BU_{\Bi} \ \By_{t-1} \  + \
    \Bb_{\Bi} \right) & \text{input gate} \\
\Bf_t \ &= \ \sigma \left( \BW_{\Bf} \ \Bx_t \  + \ \BU_{\Bf} \ \By_{t-1} \  + \
   \Bb_{\Bf} \right) & \text{forget gate} \\
\Bc_t \ &= \  \Bi_t \odot \Bz_t \ + \ 
\Bf_t \odot \Bc_{t-1} & \text{cell state} \\
\Bo_t \ &= \ \sigma \left( \BW_{\Bo} \ \Bx_t \   + \ \BU_{\Bo} \ \By_{t-1} \  + \
  \Bb_{\Bo} \right) & \text{output gate} \\
\By_t \ &= \ \Bo_t \odot h\left( \Bc_t \right) &
\text{cell output} \label{Arr:eq_end:standard_LSTM_forward}
\end{aligned}
\end{eqnarray}
\citep{Arras2019}
